A Transprecision Floating-Point Platform for Ultra-Low Power Computing

In modern low-power embedded platforms, floating-point (FP) operations emerge as a major contributor to the energy consumption of compute-intensive applications with large dynamic range. Experimental evidence shows that 50% of the energy consumed by a core and its data memory is related to FP computations. The adoption of FP formats requiring a lower number of bits is an interesting opportunity to reduce energy consumption, since it allows to simplify the arithmetic circuitry and to reduce the memory bandwidth between memory and registers by enabling vectorization. From a theoretical point of view, the adoption of multiple FP types perfectly fits with the principle of transprecision computing, allowing fine-grained control of approximation while meeting specified constraints on the precision of final results. In this paper we propose an extended FP type system with complete hardware support to enable transprecision computing on low-power embedded processors, including two standard formats (binary32 and binary16) and two new formats (binary8 and binary16alt). First, we introduce a software library that enables exploration of FP types by tuning both precision and dynamic range of program variables. Then, we present a methodology to integrate our library with an external tool for precision tuning, and experimental results that highlight the clear benefits of introducing the new formats. Finally, we present the design of a transprecision FP unit capable of handling 8-bit and 16-bit operations in addition to standard 32-bit operations. Experimental results on FP-intensive benchmarks show that up to 90% of FP operations can be safely scaled down to 8-bit or 16-bit formats. Thanks to precision tuning and vectorization, execution time is decreased by 12% and memory accesses are reduced by 27% on average, leading to a reduction of energy consumption up to 30%.

==> tex/02a_preliminaries.tex <==
\section{On Floating-Point Formats}
\label{sec:prelim}
%
Applications that operate on real-valued data most commonly use IEEE 754-compliant floating-point formats \cite{zuras2008ieee}. Of the standard formats, binary32 and binary64 enjoy the most wide-spread use and are also available on general-purpose consumer platforms. While even larger formats are commonly used for scientific computations, reducing the amount of data to process and hence the width of floating-point formats is more interesting for power-constrained and embedded platforms.
While smaller-than-\SI{32}{\bit} floating-point formats (also called \emph{minifloat}s) have seen use in computer graphics applications [TODO cite some gpu with with fp24 support or directX9], their relevance is rising with the spread of energy-constrained near-sensor processing nodes and internet-of-things endpoints.

In this work, four floating-point formats are considered and shown in Fig.~\ref{fig:formats}. The two IEEE-specified formats \emph{binary32} and \emph{binary16} are used alongside two custom formats, \emph{binary16alt} and \emph{binary8}.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{formats}
  \vspace{-0.2in}
  \caption{Overview of floating-point formats used throughout this work.}\label{fig:formats}
\end{figure}

A drawback of binary16 is that both dynamic range and precision are diminished when compared to binary32. This leads to saturation when converting values with large magnitude from binary32, disqualifying the \SI{16}{\bit} format from being used for transprecision tuning in these cases. Hence, the binary16alt format that operates on 8 exponent bits and 7 mantissa bits was added to our set of types. It features the same dynamic range as binary32, allowing the whole range of values to be converted - albeit at a much larger granularity. These conversions are especially cheap in hardware since the exponent does not need extra processing.

Similarly, the binary8 format was conceived to mirror the dynamic range of binary16, using 5 exponent and 2 mantissa bits. Again, conversions between the two formats only affect precision but do not saturate for values of large magnitudes. Additionally, operations on binary8 become very cheap in hardware since there are only two explicit mantissa bits.

The two custom formats introduced here both follow the principles of the IEEE 754 standard, namely the support and encoding of denormal numbers, infinities and NaN values. 
